Communicating Visualizations without Visuals: Investigation of Visualization Alternative Text for People with Visual Impairments

Alternative text is critical in communicating graphics to people who are blind or have low vision. Especially for graphics that contain rich information, such as visualizations, poorly written or an absence of alternative texts can worsen the information access inequality for people with visual impairments. In this work, we consolidate existing guidelines and survey current practices to inspect to what extent current practices and recommendations are aligned. Then, to gain more insight into what people want in visualization alternative texts, we interviewed 22 people with visual impairments regarding their experience with visualizations and their information needs in alternative texts. The study findings suggest that participants actively try to construct an image of visualizations in their head while listening to alternative texts and wish to carry out visualization tasks (e.g., retrieve specific values) as sighted viewers would. The study also provides ample support for the need to reference the underlying data instead of visual elements to reduce users' cognitive burden. Informed by the study, we provide a set of recommendations to compose an informative alternative text.

==> 100-alt-text.tex <==
How to add alt text using adobe acrobat
1. Choose View > Show/Hide > Navigation Panels > Tags.

2. (if there is no tags tree create one)Expand the logical structure tree to find and select the desired <Figure> tag element for the image.
3. Choose Properties from the Options menu in the Tags panel.
4. In the Object Properties dialog box, click the Tag panel.
Type text in the alternative text field that describes the figure.


Figure 1
A bar chart that shows the frequency of each component that appears in the alt texts from the ASSETS and CHI collections. 
Details of the visualization are as follows. 
From left to right, the components listed on the x axis are summary (topic), axes, data points, chart type, ticks, data trends, color, and shape. The bars go up on the y axis as high as its frequency. For example, the summary (topic) component was included in the ASSETS collections 99% of the time. There is a bar that goes up to 99% with a percentage specified on top of each of the bars. The ASSETS data is colored in blue and the CHI data is colored in red. The overall range of the individual components is from 0% to 99%. There is a decreasing trend for the ASSETS collection in the order of the components. More specifically, summary (topic) has the highest frequency at 99%, and the shape component has the lowest frequency at 0%. As for the CHI collection, it has the highest frequency for summary (topic) at 97%, then drastically decreases for components such as axes, data points, ticks, etc to around 10% to less than 20%. However, the chart type frequency is at 34%.

Figure 2
Two bar charts that shows the frequency of the top-3 most common combinations of components used in alt texts, each from the ASSETS and CHI collections. 
Details of the visualization are as follows.
There are two separate sideways bar charts. The one on the left depicts the ASSETS collection. There are different combinations on the y axis. From top to bottom, the combinations are summary, axes, ticks, data points, the next is summary, axes, ticks, data trends, data points, the last is summary. The bars extend on the x axis as much as its frequency. For example the first combination of summary, axes, ticks, data points extend to 18%, with the percentage specified next to each of the bars. The right chart depicts the CHI collection. From top to bottom, the combinations are summary, the next is summary, chart type, and the last is summary, data points. For both of the charts, the trend seems to decrease from top to bottom. For the ASSETS collection, the first combination is at 18% and the last is at 8%. For the CHI collection, the first combination is at 48% and the last is at 4%.

Figure 3
A table that shows the study stimuli. Each participant saw all of the visualizations parked with a different style of alt text. The columns from left to right contain the visualization ID, the visualization (chart type, topic), number of variables, brief description, detailed description, data trends, and data points.

Figure 4

A flowchart that shows the study procedure. The first element is as follows: a) Answer demographics questions, vision conditions, prior experience with assistive technology and visualizations. Next, b) Examine four visualization stimuli. Examine first visualization, Get detailed description, improve/refine given alt text, examine next visualization, and s on. Lastly, c) Share overall preferences, usefulnesss of each style of alt texts etc.


==> TODO.tex <==
============TODO============

============DONE============
(done) YK: phase 2 analysis and summary, shuhbam from 710 row 
(done) CJ: Capitalize the first letter of quotes
(done) CJ: alt-text > alt texts 
(done) CJ: alternative text > alt texts
(done) CJ: unify Braille > braille
add miller Amanda Miller to table 
YK:  full column figure refine, add data
CJ: functional vision?
CJ: proofread/edit phase 2
CJ: proofread/edit phase 3
CJ: write conclusion
balance participants 
explain more about thematic coding by looking at https://patron.library.wisc.edu/authn/splash?url=https://dl.acm.org/doi/epdf/10.1145/3234695.3236359
add citation for news articles that we use 
delete the chart encounter in the participant table 
YK: refine how we formulated study stimuli
BLV -> people with visual impairments, visually impaired 
YK: add one more paragraph in discussion section
CJ: proofread/edit discussion
YKL clean up the related work

============FINAL PROOF READING============
missing citation find question marks
check references to see if anything wrong
coherent usage of alt text, people with visual impairment
everything present tense except what we did

